Integrated Planning of a Solar/Storage Collective

French regulation allows consumers in low-voltage networks to form collectives to produce, share, and consume local energy under the collective self-consumption framework. A natural consequence of collectively-owned generation projects is the need to allocate production among consumers. In long-term plans, production allocation determines each of the consumers' benefits of joining the collective. In the short-term, energy should be dynamically allocated to reflect operation. This paper presents a framework that integrates long and short-term planning of a collective that shares a solar plus energy storage system. In the long-term planning stage, we maximize the collective's welfare and equitably allocate expected energy to each consumer. For operation, we propose a model predictive control algorithm that minimizes short-term costs and allocates energy to each consumer on a 30-minute basis (as required by French regulation). We adjust the energy allotment ex-post operation to reflect the materialization of uncertainty. We present a case study where we showcase the framework for a 15 consumer collective.

==> Self-consumption project - Arxiv/Data/data.tex <==
















==> Self-consumption project - Arxiv/Data/data_mismatch.tex <==







==> Self-consumption project - Arxiv/Data/data_mismatch_myopic.tex <==



==> Self-consumption project - Arxiv/Data/data_mismatch_myopic_rule-based.tex <==



==> Self-consumption project - Arxiv/Data/data_solar_sensitivity.tex <==



==> Self-consumption project - Arxiv/Figures/flowchart.tex <==
\begin{figure}
\includegraphics[width=0.4\linewidth]{Figures/flowchart_3.pdf}
\centering
\caption{Diagram representing the framework proposed in this paper.}
\label{fig: outline}
\end{figure}

==> Self-consumption project - Arxiv/Tables/table_benefit_split.tex <==
\begin{table}[ht]
    \caption{Investor profit and consumer savings under different prices for both the baseline and the optimistic cases.}
\textbf{\underline{Pessimistic case}} 
  \begin{center}
\begin{tabular}{c|c|c|c} 
\textbf{$\boldsymbol{p}$ (\faEuro/kWh)} & $\boldsymbol{\gamma}$ & \textbf{\begin{tabular}[c]{@{}c@{}} investor profit (k\faEuro) \end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}  consumer  savings (k\faEuro) \end{tabular}}} \\
\hline
0.10             & 0              & 0                                                                               & {\color[HTML]{009901}32 }                                                                                                           \\ 
0.115             & 0.5            & {\color[HTML]{009901}16 }                                                                             & {\color[HTML]{009901}16   }                                                                                                           \\ 
0.13             & 1              & {\color[HTML]{009901}32  }                                                                           & 0                                                                                                               \\ 
\end{tabular}

\end{center}
\textbf{\underline{Baseline case}} 
  \begin{center}
\begin{tabular}{c|c|c|c} 
\textbf{$\boldsymbol{p}$ (\faEuro/kWh)} & $\boldsymbol{\gamma}$ & \textbf{\begin{tabular}[c]{@{}c@{}} investor profit (k\faEuro) \end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}  consumer  savings (k\faEuro) \end{tabular}}} \\
\hline
0.05             & 0              & 0                                                                               & {\color[HTML]{009901}142 }                                                                                                           \\ 
0.09             & 0.5            & {\color[HTML]{009901}71 }                                                                             & {\color[HTML]{009901}71   }                                                                                                           \\ 
0.13             & 1              & {\color[HTML]{009901}142  }                                                                           & 0                                                                                                               \\ 
\end{tabular}
\end{center}

    \label{table:benefit_split}
    
\end{table}




==> Self-consumption project - Arxiv/Tables/table_cost_benefits.tex <==
\begin{table}[ht]
\caption{Expected costs, benefit, and net benefit in both cases.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{costs (k\faEuro)}}               & \multicolumn{3}{c|}{\textbf{benefit (k\faEuro)}}                                          &                                                                                       \\ \cline{1-5}
\textbf{CapEx}             & \textbf{OpEx}             & \textbf{grid savings}      & \textbf{subsidy}         & \textbf{surplus}           & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}net benefit \\ (k\faEuro)\end{tabular}}} \\ \hline
\multicolumn{6}{|c|}{\textbf{baseline case}}                                                                                                                                                                                      \\ \hline
{\color[HTML]{CB0000} 258} & {\color[HTML]{CB0000} 86} & {\color[HTML]{009901} 224} & 0                        & {\color[HTML]{009901} 262} & {\color[HTML]{009901} 142}                                                            \\ \hline
\multicolumn{6}{|c|}{\textbf{pessimistic case}}                                                                                                                                                                                     \\ \hline
{\color[HTML]{CB0000} 110} & {\color[HTML]{CB0000} 10} & {\color[HTML]{009901} 148} & {\color[HTML]{009901} 5} & 0                          & {\color[HTML]{009901} 32}                                                             \\ \hline
\end{tabular}
\end{center}
\label{table:cost_benefits}
\end{table}

